ValuePilot: A Two-Phase Framework for Value-Driven Decision-Making

Despite recent advances in artificial intelligence (AI), it poses challenges to ensure personalized decision-making in tasks that are not considered in training datasets. To address this issue, we propose ValuePilot, a two-phase value-driven decision-making framework comprising a dataset generation toolkit DGT and a decision-making module DMM trained on the generated data. DGT is capable of generating scenarios based on value dimensions and closely mirroring real-world tasks, with automated filtering techniques and human curation to ensure the validity of the dataset. In the generated dataset, DMM learns to recognize the inherent values of scenarios, computes action feasibility and navigates the trade-offs between multiple value dimensions to make personalized decisions. Extensive experiments demonstrate that, given human value preferences, our DMM most closely aligns with human decisions, outperforming Claude-3.5-Sonnet, Gemini-2-flash, Llama-3.1-405b and GPT-4o. This research is a preliminary exploration of value-driven decision-making. We hope it will stimulate interest in value-driven decision-making and personalized decision-making within the community.

==> sections/1_introduction_old.tex <==
As artificial intelligence (AI) systems become increasingly integrated into human environments, their ability to make intelligent, adaptive, and human-like decisions is critical \citep{lake2017building}. Traditional AI decision-making primarily optimizes for efficiency or goal completion, often overlooking the complex, value-driven nature of human choices \citep{mekni2021artificial, xu2021human}. In real-world scenarios, human decision-making is shaped not just by objective outcomes but also by deeply held value dimensions, such as fairness, curiosity, safety, etc. Furthermore, decisions are inherently individualized, as different people prioritize different values in similar contexts. The challenge, then, is to develop AI agents that can internalize human value structures and make personalized, context-aware decisions that reflect individual differences.

% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/pipeline1.jpg}
%     \caption{ValuePilot framework. The ValuePilot framework simulates individual preferences and guides AI decision-making through a two-phase process. In the first phase, key value dimensions are extracted and utilized by \textbf{VP-DataGT} to generate a structured training dataset, which includes scenario descriptions, potential actions, and corresponding value dimension scores. In the second phase, the trained \textbf{VP-DeciMN} module uses these inputs, along with preferences modeled by the value dimensions, to rank the possible actions.}
%     \label{fig:Pipeline}
%     \vspace{-14pt}
% \end{figure}

Human decision-making is inherently value-driven, a principle well-established in psychology and cognitive science. Schwartz’s theory of basic human values \citep{schwartz2012overview} describes a universal structure of values that shape human choices, while Maslow’s hierarchy of needs \citep{maslow1943theory} explains how fundamental and higher-order values influence behavior. These perspectives emphasize that decision-making is not purely about optimizing outcomes but involves balancing competing values in different contexts.

Existing AI approaches to value alignment, such as reinforcement learning from human feedback (RLHF) \citep{christiano2017deep} and direct preference optimization (DPO) \citep{rafailov2024direct}, attempt to align AI behavior with broad human preferences. However, these methods treat human values as a single, collective entity, failing to account for individual variations in value priorities. Similarly, structured decision-making models like AutoPlan \citep{ouyang2023autoplan} and ReAct \citep{yao2022react} focus on optimizing task efficiency while neglecting personalized, value-driven motivations. To develop AI that can reason and act like a human, it must not only recognize universal human values but also adapt decisions to individual value preferences.

While value-driven reasoning provides a foundation for human-like decision-making, personalization is essential for AI to interact meaningfully with individuals. Different people assign different weights to value dimensions, shaping how they navigate trade-offs in decision-making. For example, one person may prioritize curiosity over safety, while another may favor caution in the same scenario. Capturing these differences requires AI to model value dimensions and adjust decisions based on individual preferences.

However, personalized decision-making is inherently complex due to multiple interacting factors: Each action must be evaluated based on how it aligns with relevant values; the scenario context must be considered, ensuring that decisions are environment-sensitive rather than isolated choices; the individual’s value preferences must be integrated to balance objective action feasibility with subjective personal alignment.

This complexity makes fine-grained preference modeling particularly challenging, especially in the absence of high-quality, structured training data. Existing datasets for decision-making tasks, such as ALFWorld \citep{shridhar2020alfworld} and InterCode \citep{yang2024intercode}, focus on task completion rather than modeling human value trade-offs, making them unsuitable for training AI agents in value-driven decision-making.

To address this gap, we propose a structured dataset generation method that models how value dimensions influence decision-making. Our approach constructs a multi-dimensional value space, numerically evaluating each action based on its alignment with predefined values to capture human-like trade-offs. Unlike traditional supervised learning focused on task performance, our method integrates value-based reasoning, enabling AI to internalize decision patterns rather than merely optimizing objectives. This framework not only generates a dataset but also provides a scalable methodology for producing diverse, value-driven decision-making data.

To enable value-driven and personalized AI decision-making, we propose \textbf{ValuePilot}, a two-phase framework for value-driven decision-making that enables AI agents to make deeply personalized decisions, reflecting individual preferences of every human value. Unlike prior work, ValuePilot:
\begin{enumerate}
    \vspace{-4mm}
    \item Learns individual value preferences rather than generalizing across a collective human model.
    \vspace{-4mm}
    \item Generates a structured dataset using GPT-4, with numerical annotations that quantify the influence of each action on value dimensions.
    \vspace{-4mm}
    \item Optimizes decision-making through value-based ranking, allowing agents to balance personalized preferences with environmental context.
\end{enumerate}
\vspace{-3mm}
% Our method consists of two key phases (shown in Figure \ref{fig:Pipeline}):

% \textbf{Phase 1: ValuePilot Dataset Generation Toolkit (VP-DataGT)} 
% This phase constructs a structured dataset to model human decision-making across different value dimensions. Using GPT-4, VP-DataGT generates scenario descriptions, candidate actions, and corresponding value scores. Automated filtering ensures data consistency and balance. The output is a dataset that captures diverse human preferences.

% \textbf{Phase 2: ValuePilot Decision Making Networks (VP-DeciMN)} 
% A T5 encoder is fine-tuned to map textual descriptions to latent value representations. The model ranks actions based on their alignment with individual value preferences and contextual factors, producing personalized decision outputs.

By bridging value-based reasoning and personalized decision-making, our approach advances beyond traditional value alignment and task-driven optimization, providing a scalable solution for training AI agents capable of context-aware, human-aligned, and individually tailored decisions.
